On The Complexity of Maximizing Temporal Reachability via Trip Temporalisation

We consider the problem of assigning appearing times to the edges of a digraph in order to maximize the (average) temporal reachability between pairs of nodes. Motivated by the application to public transit networks, where edges cannot be scheduled independently one of another, we consider the setting where the edges are grouped into certain walks (called trips) in the digraph and where assigning the appearing time to the first edge of a trip forces the appearing times of the subsequent edges. In this setting, we show that, quite surprisingly, it is NP-complete to decide whether there exists an assignment of times connecting a given pair of nodes. This result allows us to prove that the problem of maximising the temporal reachability cannot be approximated within a factor better than some polynomial term in the size of the graph. We thus focus on the case where, for each pair of nodes, there exists an assignment of times such that one node is reachable from the other. We call this property strong temporalisability. It is a very natural assumption for the application to public transit networks. On the negative side, the problem of maximising the temporal reachability remains hard to approximate within a factor $\sqrt$ n/12 in that setting. Moreover, we show the existence of collections of trips that are strongly temporalisable but for which any assignment of starting times to the trips connects at most an O(1/ $\sqrt$ n) fraction of all pairs of nodes. On the positive side, we show that there must exist an assignment of times that connects a constant fraction of all pairs in the strongly temporalisable and symmetric case, that is, when the set of trips to be scheduled is such that, for each trip, there is a symmetric trip visiting the same nodes in reverse order. Keywords:edge labeling edge scheduled network network optimisation temporal graph temporal path temporal reachability time assignment

==> img/clausegadget.tex <==
\SetVertexStyle[FillColor=white]
\SetEdgeStyle[Color=black]
\begin{tikzpicture}
  \Vertex[x=0,y=0,label=$w_{j}$,size=0.7]{wj}
  \Vertex[x=2,y=1,label=$l_j^1$,size=0.7]{lj1}
  \Vertex[x=2,y=0,label=$l_j^2$,size=0.7]{lj2}
  \Vertex[x=2,y=-1,label=$l_j^3$,size=0.7]{lj3}
  \Vertex[x=4,y=0,label=$w_{j+1}$,size=0.7]{wjp1}
  \Edge[Direct](wj)(lj1)
  \Edge[Direct](wj)(lj2)
  \Edge[Direct](wj)(lj3)
  \Edge[Direct](lj1)(wjp1)
  \Edge[Direct](lj2)(wjp1)
  \Edge[Direct](lj3)(wjp1)
\end{tikzpicture}


==> img/introduction/edgetemporalisation.tex <==
\SetVertexStyle[FillColor=white]
\SetEdgeStyle[Color=black]
\begin{tikzpicture}[x=2cm,y=2cm]
  \Vertex[x=0,y=0,label=$x$,size=0.5]{x}
  \Vertex[x=0,y=2,label=$y$,size=0.5]{y}
  \Vertex[x=2,y=2,label=$w$,size=0.5]{w}
  \Vertex[x=2,y=0,label=$z$,size=0.5]{z}
%
  \Edge[Direct,label=$2$,position=left](x)(y)
  \Edge[Direct,bend=30,label={~$2$~},position=above](y)(w)
  \Edge[Direct,bend=-30,label={~$1$~},position=below](y)(w)
  \Edge[Direct,label=$2$,position=right](w)(z)
  \Edge[Direct,label={~$1$~},position=below](z)(x)
\end{tikzpicture}
\qquad
\begin{tikzpicture}[x=2cm,y=2cm]
  \Vertex[x=0,y=0,label=$x$,size=0.5]{x}
  \Vertex[x=0,y=2,label=$y$,size=0.5]{y}
  \Vertex[x=2,y=2,label=$w$,size=0.5]{w}
  \Vertex[x=2,y=0,label=$z$,size=0.5]{z}
%
  \Edge[Direct,label={$5,2$},position=left](x)(y)
  \Edge[Direct,bend=30,label={$7,2$},position=above](y)(w)
  \Edge[Direct,bend=-30,label={$1,1$},position=below](y)(w)
  \Edge[Direct,label={$2,2$},position=right](w)(z)
  \Edge[Direct,label={$4,1$},position=below](z)(x)
\end{tikzpicture}
\qquad
\begin{tikzpicture}[x=2cm,y=2cm]
  \Vertex[x=0,y=0,label=$x$,size=0.5]{x}
  \Vertex[x=0,y=2,label=$y$,size=0.5]{y}
  \Vertex[x=2,y=2,label=$w$,size=0.5]{w}
  \Vertex[x=2,y=0,label=$z$,size=0.5]{z}
%
  \Edge[Direct,label={$5,2$},position=left](x)(y)
  \Edge[Direct,bend=30,label={$1,2$},position=above](y)(w)
  \Edge[Direct,bend=-30,label={$7,1$},position=below](y)(w)
  \Edge[Direct,label={$2,2$},position=right](w)(z)
  \Edge[Direct,label={$4,1$},position=below](z)(x)
\end{tikzpicture}

==> img/mroett/reduction.tex <==
\SetVertexStyle[FillColor=white]
\SetEdgeStyle[Color=black]
\begin{tikzpicture}[x=2cm,y=2cm,scale=0.8, every node/.style={scale=0.8}]
  \tikzmath{\xd=2;\yd=2;\gd=2;\xcd=4;\ycd=2;\ykd=1;\yud=2;\xad=2;\yad=1;\xf1=0;\xt1=\xf1+\xd;\y1=0;\y2=\y1+\yd;\xf2=\xt1+\gd;\xt2=\xf2+\xd;\xf3=\xt2+\gd;\xt3=\xf3+\xd;\xc1=1;\xc2=\xc1+\xcd;\xc3=\xc2+\xcd;\yc1=\y1-\ycd;\yc2=\y2+\ycd;\yk1=\yc1-\ykd;\yk2=\yc2+\ykd;\xk1=\xf1+\xd/2;\xk2=\xf2+\xd/2;\xk3=\xf3+\xd/2;\yu1=\yk1-\yud;\yu2=\yk2+\yud;\xb1=\xt3+\xad;\xa2=\xb1+3*\xad/4;\xa3=\xa2+3*\xad/4;\ya=\y1+\yd/2;}
  \Vertex[x=\xf1,y=\y1,label=$f_{1}^{1}$,size=0.5]{f11}
  \Vertex[x=\xf1,y=\y2,label=$t_{1}^{2}$,size=0.5]{f12}
  \Vertex[x=\xt1,y=\y1,label=$t_{1}^{1}$,size=0.5]{t11}
  \Vertex[x=\xt1,y=\y2,label=$f_{1}^{2}$,size=0.5]{t12}
%
  \Vertex[x=\xf2,y=\y1,label=$f_{2}^{1}$,size=0.5]{f21}
  \Vertex[x=\xf2,y=\y2,label=$t_{2}^{2}$,size=0.5]{f22}
  \Vertex[x=\xt2,y=\y1,label=$t_{2}^{1}$,size=0.5]{t21}
  \Vertex[x=\xt2,y=\y2,label=$f_{2}^{2}$,size=0.5]{t22}
%
  \Vertex[x=\xf3,y=\y1,label=$f_{3}^{1}$,size=0.5]{f31}
  \Vertex[x=\xf3,y=\y2,label=$t_{3}^{2}$,size=0.5]{f32}
  \Vertex[x=\xt3,y=\y1,label=$t_{3}^{1}$,size=0.5]{t31}
  \Vertex[x=\xt3,y=\y2,label=$f_{3}^{2}$,size=0.5]{t32}
%
  \Vertex[x=\xc1,y=\yc1,label=$c_{1}^{1}$,size=0.5]{c11}
  \Vertex[x=\xc2,y=\yc1,label=$c_{2}^{1}$,size=0.5]{c21}
  \Vertex[x=\xc3,y=\yc1,label=$c_{3}^{1}$,size=0.5]{c31}
%
  \Vertex[x=\xc1,y=\yc2,label=$c_{1}^{2}$,size=0.5]{c12}
  \Vertex[x=\xc2,y=\yc2,label=$c_{2}^{2}$,size=0.5]{c22}
  \Vertex[x=\xc3,y=\yc2,label=$c_{3}^{2}$,size=0.5]{c32}
%
  \Vertex[x=\xf1,y=\yk1,label=$d_{1}^{1}$,size=0.5]{d11}
  \Vertex[Pseudo,x=\xk1,y=\yk1,label=$\cdots$,size=0.5, opacity=0]{ddots1}
  \Vertex[x=\xt1,y=\yk1,label=$d_{1}^{K}$,size=0.5]{d1K}
%
  \Vertex[x=\xf2,y=\yk1,label=$d_{2}^{1}$,size=0.5]{d21}
  \Vertex[Pseudo,x=\xk2,y=\yk1,label=$\cdots$,size=0.5, opacity=0]{ddots2}
  \Vertex[x=\xt2,y=\yk1,label=$d_{2}^{K}$,size=0.5]{d2K}
%
  \Vertex[x=\xf3,y=\yk1,label=$d_{3}^{1}$,size=0.5]{d31}
  \Vertex[Pseudo,x=\xk3,y=\yk1,label=$\cdots$,size=0.5, opacity=0]{ddots3}
  \Vertex[x=\xt3,y=\yk1,label=$d_{3}^{K}$,size=0.5]{d3K}
%
  \Vertex[x=\xf1,y=\yk2,label=$e_{1}^{1}$,size=0.5]{e11}
  \Vertex[Pseudo,x=\xk1,y=\yk2,label=$\cdots$,size=0.5, opacity=0]{edots1}
  \Vertex[x=\xt1,y=\yk2,label=$e_{1}^{K}$,size=0.5]{e1K}
%
  \Vertex[x=\xf2,y=\yk2,label=$e_{2}^{1}$,size=0.5]{e21}
  \Vertex[Pseudo,x=\xk2,y=\yk2,label=$\cdots$,size=0.5, opacity=0]{edots2}
  \Vertex[x=\xt2,y=\yk2,label=$e_{2}^{K}$,size=0.5]{e2K}
%
  \Vertex[x=\xf3,y=\yk2,label=$e_{3}^{1}$,size=0.5]{e31}
  \Vertex[Pseudo,x=\xk3,y=\yk2,label=$\cdots$,size=0.5, opacity=0]{edots3}
  \Vertex[x=\xt3,y=\yk2,label=$e_{3}^{K}$,size=0.5]{e3K}
%
  \Vertex[x=\xf2,y=\yu1,label=$u_{2}$,size=0.5]{u2}
  \Vertex[x=\xt2,y=\yu1,label=$u_{1}$,size=0.5]{u1}
%
  \Vertex[x=\xf2,y=\yu2,label=$u_{3}$,size=0.5]{u3}
  \Vertex[x=\xt2,y=\yu2,label=$u_{4}$,size=0.5]{u4}
%
  \Vertex[x=\xb1,y=\ya,label=$b_{1}$,size=0.5]{b1}
  \Vertex[Pseudo,x=\xa2,y=\ya,label=$\cdots$,size=0.5, opacity=0]{adots}
  \Vertex[x=\xa3,y=\ya,label=$b_{M}$,size=0.5]{bM}
%
  \Edge[Direct](t11)(t12)
  \Edge[Direct](t12)(f11)
  \Edge[Direct](f11)(f12)
  \Edge[Direct](f12)(t11)
%
  \Edge[Direct](t21)(t22)
  \Edge[Direct](t22)(f21)
  \Edge[Direct](f21)(f22)
  \Edge[Direct](f22)(t21)
%
  \Edge[Direct](t31)(t32)
  \Edge[Direct](t32)(f31)
  \Edge[Direct](f31)(f32)
  \Edge[Direct](f32)(t31)
%
  \Edge[Direct](c11)(t11)
  \Edge[Direct](c11)(t21)
  \Edge[Direct](c11)(t31)
%
  \Edge[Direct](c21)(f11)
  \Edge[Direct](c21)(t21)
  \Edge[Direct](c21)(t31)
%
  \Edge[Direct](c31)(f11)
  \Edge[Direct](c31)(f21)
  \Edge[Direct](c31)(f31)
%
  \Edge[Direct](f12)(c12)
  \Edge[Direct](f22)(c12)
  \Edge[Direct](f32)(c12)
%
  \Edge[Direct](t12)(c22)
  \Edge[Direct](f22)(c22)
  \Edge[Direct](f32)(c22)
%
  \Edge[Direct](t12)(c32)
  \Edge[Direct](t22)(c32)
  \Edge[Direct](t32)(c32)
%
  \Edge[Direct](d11)(c11)
  \Edge[Direct](d1K)(c11)
%
  \Edge[Direct](d21)(c21)
  \Edge[Direct](d2K)(c21)
%
  \Edge[Direct](d31)(c31)
  \Edge[Direct](d3K)(c31)
%
  \Edge[Direct](c12)(e11)
  \Edge[Direct](c12)(e1K)
%
  \Edge[Direct](c22)(e21)
  \Edge[Direct](c22)(e2K)
%
  \Edge[Direct](c32)(e31)
  \Edge[Direct](c32)(e3K)
%
  \Edge[Direct](u1)(u2)
  \Edge[Direct](u2)(d11)
  \Edge[Direct](u2)(d1K)
  \Edge[Direct](u2)(d21)
  \Edge[Direct](u2)(d2K)
  \Edge[Direct](u2)(d31)
  \Edge[Direct](u2)(d3K)
%
  \Edge[Direct](u3)(u4)
  \Edge[Direct](e11)(u3)
  \Edge[Direct](e1K)(u3)
  \Edge[Direct](e21)(u3)
  \Edge[Direct](e2K)(u3)
  \Edge[Direct](e31)(u3)
  \Edge[Direct](e3K)(u3)
%
%   \Vertex[x=12,y=-3,Pseudo,size=0,opacity=0]{dum1}
%   \Edge(b1)(dum1)
  \Edge[Direct,bend=45](b1)(u1)
  \Edge[Direct,bend=45](bM)(u1)
%   \draw[line width=1.5pt,fill=black] (b1)--(6,-1.5);
%   \draw[-latex,line width=1.5pt,fill=black] (6,-1.5)--(u1);
%   \draw[line width=1.5pt,fill=black] (bM)--(7.5,-2);
%   \draw[-latex,line width=1.5pt,fill=black] (7.5,-2)--(u1);
%
  \Edge[Direct,bend=45](u4)(b1)
  \Edge[Direct,bend=45](u4)(bM)
%   \draw[line width=1.5pt,fill=black] (u4)--(6,2.5);
%   \draw[-latex,line width=1.5pt,fill=black] (6,2.5)--(b1);
%   \draw[line width=1.5pt,fill=black] (u4)--(7.5,3);
%   \draw[-latex,line width=1.5pt,fill=black] (7.5,3)--(bM);
%
  \Edge[Direct,style={dashed}](c11)(c22) 
  \Edge[Direct,style={dashed}](c11)(c32) 
  \Edge[Direct,style={dashed}](c21)(c12) 
  \Edge[Direct,style={dashed}](c21)(c32) 
  \Edge[Direct,style={dashed}](c31)(c12) 
  \Edge[Direct,style={dashed}](c31)(c22) 
\end{tikzpicture}


==> img/reductionexample.tex <==
\SetVertexStyle[FillColor=white]
\SetEdgeStyle[Color=black]
\begin{tikzpicture}
  \Vertex[x=0,y=0,label=$v_{1}$]{v1}
  \Vertex[x=1.5,y=1,label=$f_1^1$]{f11}
  \Vertex[x=1,y=-1,label=$t_1^1$]{t11}
  \Vertex[x=2,y=-1,label=$t_1^2$]{t12}
  \Vertex[x=3,y=0,label=$v_2$]{v2}
  %
  \Vertex[x=4,y=1,label=$f_2^1$]{f21}
  \Vertex[x=5,y=1,label=$f_2^2$]{f22}
  \Vertex[x=4.5,y=-1,label=$t_2^1$]{t21}
  \Vertex[x=6,y=0,label=$v_3$]{v3}
  %
  \Vertex[x=7.5,y=1,label=$f_3^1$]{f31}
  \Vertex[x=7,y=-1,label=$t_3^1$]{t31}
  \Vertex[x=8,y=-1,label=$t_3^2$]{t32}
  \Vertex[x=9,y=0,label=$v_4$]{v4}
  %
  \Vertex[x=10,y=0,label=$w_1$]{w1}
  %
  \Vertex[x=11,y=1,label=$l_1^1$]{l11}
  \Vertex[x=11,y=0,label=$l_1^2$]{l12}
  \Vertex[x=11,y=-1,label=$l_1^3$]{l13}
  \Vertex[x=12,y=0,label=$w_2$]{w2}
  %
  \Vertex[x=13,y=1,label=$l_2^1$]{l21}
  \Vertex[x=13,y=0,label=$l_2^2$]{l22}
  \Vertex[x=13,y=-1,label=$l_2^3$]{l23}
  \Vertex[x=14,y=0,label=$w_3$]{w3}
  %
  \Vertex[x=15,y=1,label=$l_3^1$]{l31}
  \Vertex[x=15,y=0,label=$l_3^2$]{l32}
  \Vertex[x=15,y=-1,label=$l_3^3$]{l33}
  \Vertex[x=16,y=0,label=$w_4$]{w4}
  %
  \Edge[Direct](v1)(f11)
  \Edge[Direct](v1)(t11)
  \Edge[Direct,color=red,style={dashed}](t11)(t12)
  \Edge[Direct,color=red](f11)(v2)
  \Edge[Direct,color=red,style={dotted}](t12)(v2)
  %
  \Edge[Direct](v2)(f21)
  \Edge[Direct](v2)(t21)
  \Edge[Direct,color=blue](f21)(f22)
  \Edge[Direct,color=blue,style={dashed}](f22)(v3)
  \Edge[Direct,color=blue,style={dotted}](t21)(v3)
  %
  \Edge[Direct](v3)(f31)
  \Edge[Direct](v3)(t31)
  \Edge[Direct,color=green](t31)(t32)
  \Edge[Direct,color=green,style={dashed}](f31)(v4)
  \Edge[Direct,color=green,style={dotted}](t32)(v4)
  %
  \Edge[Direct](v4)(w1)
  %
  \Edge[Direct,color=red](w1)(l11)
  \Edge[Direct,color=blue](w1)(l12)
  \Edge[Direct,color=green](w1)(l13)
  \Edge[Direct](l11)(w2)
  \Edge[Direct](l12)(w2)
  \Edge[Direct](l13)(w2)
  %
  \Edge[Direct,color=red,style={dashed}](w2)(l21)
  \Edge[Direct,color=blue,style={dashed}](w2)(l22)
  \Edge[Direct,color=green,style={dashed}](w2)(l23)
  \Edge[Direct](l21)(w3)
  \Edge[Direct](l22)(w3)
  \Edge[Direct](l23)(w3)
  %
  \Edge[Direct,color=red,style={dotted}](w3)(l31)
  \Edge[Direct,color=blue,style={dotted}](w3)(l32)
  \Edge[Direct,color=green,style={dotted}](w3)(l33)
  \Edge[Direct](l31)(w4)
  \Edge[Direct](l32)(w4)
  \Edge[Direct](l33)(w4)
  %
  \Edge[Direct,bend=-45,color=red](l11)(f11)
  \Edge[Direct,bend=-45,color=blue](l12)(f21)
  \Edge[Direct,bend=45,color=green](l13)(t31)
  %
  \Edge[Direct,bend=-45,color=red,style={dashed}](l21)(t11)
  \Edge[Direct,bend=-45,color=blue,style={dashed}](l22)(f22)
  \Edge[Direct,bend=45,color=green,style={dashed}](l23)(f31)
  %
  \Edge[Direct,bend=-60,color=red,style={dotted}](l31)(t12)
  \Edge[Direct,bend=-50,color=blue,style={dotted}](l32)(t21)
  \Edge[Direct,bend=45,color=green,style={dotted}](l33)(t32)
\end{tikzpicture}

==> img/ssmrtt/multidigraph.tex <==
\SetVertexStyle[FillColor=white,MinSize=0.7\DefaultUnit]
\begin{tikzpicture}[font=\large\sffamily]
\node[thick,cloud, cloud puffs=15, cloud ignores aspect, minimum width=7cm, minimum height=5cm, align=center, draw] (cloud) at (0cm, 0.2cm) {};
\node at (0,-1) {($D=(V,E),\mbox{$\mathbb{T}$}$)};
\Vertex[x=-4,y=0,label=$s'$]{sprime}
\Vertex[x=-3,y=0,label=$s$]{s}
\Vertex[x=-2,y=0,label=$u_2$]{u2}
\Vertex[x=-1,y=0,label=$u_3$]{u3}
\Vertex[x=0,y=0,label=$\cdots$,style={color=white},size=0.4]{ui}
\Vertex[x=1,y=0,label=$u_{n-2}$]{un-2}
\Vertex[x=2,y=0,label=$u_{n-1}$]{un-1}
\Vertex[x=3,y=0,label=$t$]{t}
\Vertex[x=4,y=0,label=$a_{1}$]{a1}
\Vertex[x=4,y=1,label=$a_{2}$]{a2}
\Vertex[x=4,y=2,label=$\cdots$,style={color=white},size=0.4]{ai}
\Vertex[x=4,y=3,label=$a_{K-1}$]{aK-1}
\Vertex[x=4,y=4,label=$a_{K}$]{aK}
\Vertex[x=6,y=0,label=$b_{1}$]{b1}
\Vertex[x=6,y=1,label=$b_{2}$]{b2}
\Vertex[x=6,y=2,label=$\cdots$,style={color=white},size=0.4]{bi}
\Vertex[x=6,y=3,label=$b_{K-1}$]{bK-1}
\Vertex[x=6,y=4,label=$b_{K}$]{bK}
\Edge (s)(sprime)
\Edge (s)(u2)
\Edge (u2)(u3)
\Edge (u3)(ui)
\Edge (ui)(un-2)
\Edge (un-2)(un-1)
\Edge (un-1)(t)
\Edge (t)(a1)
\Edge (a1)(a2)
\Edge (a2)(ai)
\Edge (ai)(aK-1)
\Edge (aK-1)(aK)
\Edge[Direct,bend=-20](aK)(s)
\Edge (aK)(b1)
\Edge (b1)(b2)
\Edge (b2)(bi)
\Edge (bi)(bK-1)
\Edge (bK-1)(bK)
\Edge[Direct,bend=-45](bK)(s)
\Edge[Direct,bend=-45](t)(b1)
\end{tikzpicture}

==> img/ssmrtt/trips.tex <==
\SetVertexStyle[FillColor=white,MinSize=0.7\DefaultUnit]
\begin{tikzpicture}[font=\large\sffamily,scale=0.5, every node/.style={scale=0.5}]
\begin{scope}[xshift=0cm,yshift=0cm]
\Vertex[x=-1,y=0,label={$T_{A}$},style={color=white},size=1]{}
\Vertex[x=0,y=0,label=$t$,style={color=gray!30}]{t}
\Vertex[x=1.5,y=0,label=$a_{1}$]{a1}
\Vertex[x=3,y=0,label=$a_{2}$]{a2}
\Vertex[x=4.5,y=0,label=$\cdots$,style={color=white},size=0.4]{ai}
\Vertex[x=6,y=0,label=$a_{K-1}$]{aK-1}
\Vertex[x=7.5,y=0,label=$a_{K}$]{aK}
\Vertex[x=9,y=0,label=$s$]{s}
\Vertex[x=10.5,y=0,label=$u_2$]{u2}
\Vertex[x=12,y=0,label=$u_3$]{u3}
\Vertex[x=13.5,y=0,label=$\cdots$,style={color=white},size=0.4]{ui}
\Vertex[x=15,y=0,label=$u_{n-2}$]{un-2}
\Vertex[x=16.5,y=0,label=$u_{n-1}$]{un-1}
\Edge[Direct](t)(a1)
\Edge[Direct](a1)(a2)
\Edge[Direct](a2)(ai)
\Edge[Direct](ai)(aK-1)
\Edge[Direct](aK-1)(aK)
\Edge[Direct](aK)(s)
\Edge[Direct](s)(u2)
\Edge[Direct](u2)(u3)
\Edge[Direct](u3)(ui)
\Edge[Direct](ui)(un-2)
\Edge[Direct](un-2)(un-1)
\Edge[Direct,bend=-20](un-1)(t)
\end{scope}

\begin{scope}[xshift=0cm,yshift=-3cm]
\Vertex[x=-1,y=0,label={$T_{B}$},style={color=white},size=1]{}
\Vertex[x=0,y=0,label=$t$,style={color=gray!30}]{t}
\Vertex[x=1.5,y=0,label=$b_{1}$]{b1}
\Vertex[x=3,y=0,label=$b_{2}$]{b2}
\Vertex[x=4.5,y=0,label=$\cdots$,style={color=white},size=0.4]{bi}
\Vertex[x=6,y=0,label=$b_{K-1}$]{bK-1}
\Vertex[x=7.5,y=0,label=$b_{K}$]{bK}
\Vertex[x=9,y=0,label=$s$]{s}
\Vertex[x=10.5,y=0,label=$u_2$]{u2}
\Vertex[x=12,y=0,label=$u_3$]{u3}
\Vertex[x=13.5,y=0,label=$\cdots$,style={color=white},size=0.4]{ui}
\Vertex[x=15,y=0,label=$u_{n-2}$]{un-2}
\Vertex[x=16.5,y=0,label=$u_{n-1}$]{un-1}
\Edge[Direct](t)(b1)
\Edge[Direct](b1)(b2)
\Edge[Direct](b2)(bi)
\Edge[Direct](bi)(bK-1)
\Edge[Direct](bK-1)(bK)
\Edge[Direct](bK)(s)
\Edge[Direct](s)(u2)
\Edge[Direct](u2)(u3)
\Edge[Direct](u3)(ui)
\Edge[Direct](ui)(un-2)
\Edge[Direct](un-2)(un-1)
\Edge[Direct,bend=-20](un-1)(t)
\end{scope}

\begin{scope}[xshift=0cm,yshift=-5cm]
\Vertex[x=-1,y=0,label={$T_{C}$},style={color=white},size=1]{}
\Vertex[x=0,y=0,label=$s$,style={color=gray!20}]{s}
\Vertex[x=1.5,y=0,label=$u_{2}$]{u2}
\Vertex[x=3,y=0,label=$\cdots$,style={color=white},size=0.4]{ui}
\Vertex[x=4.5,y=0,label=$u_{n-1}$]{un-1}
\Vertex[x=6,y=0,label=$t$]{t}
\Vertex[x=7.5,y=0,label=$a_{1}$]{a1}
\Vertex[x=9,y=0,label=$a_{2}$]{a2}
\Vertex[x=10.5,y=0,label=$\cdots$,style={color=white},size=0.4]{ai}
\Vertex[x=12,y=0,label=$a_{K-1}$]{aK-1}
\Vertex[x=13.5,y=0,label=$a_{K}$]{aK}
\Vertex[x=15,y=0,label=$b_{1}$]{b1}
\Vertex[x=16.5,y=0,label=$b_{2}$]{b2}
\Vertex[x=18,y=0,label=$\cdots$,style={color=white},size=0.4]{bi}
\Vertex[x=19.5,y=0,label=$b_{K-1}$]{bK-1}
\Vertex[x=21,y=0,label=$b_{K}$]{bK}
\begin{scope}[yshift=-1.5cm]
\Vertex[x=15,y=0,label=$b_{1}$]{b1r}
\Vertex[x=16.5,y=0,label=$b_{2}$]{b2r}
\Vertex[x=18,y=0,label=$\cdots$,style={color=white},size=0.4]{bir}
\Vertex[x=19.5,y=0,label=$b_{K-1}$]{bK-1r}
\Vertex[x=7.5,y=0,label=$a_{1}$]{a1r}
\Vertex[x=9,y=0,label=$a_{2}$]{a2r}
\Vertex[x=10.5,y=0,label=$\cdots$,style={color=white},size=0.4]{air}
\Vertex[x=12,y=0,label=$a_{K-1}$]{aK-1r}
\Vertex[x=13.5,y=0,label=$a_{K}$]{aKr}
\Vertex[x=1.5,y=0,label=$u_{2}$]{u2r}
\Vertex[x=3,y=0,label=$\cdots$,style={color=white},size=0.4]{uir}
\Vertex[x=4.5,y=0,label=$u_{n-1}$]{un-1r}
\Vertex[x=6,y=0,label=$t$]{tr}
\Vertex[x=0,y=0,label=$s$]{sr}
\Vertex[x=-1.5,y=0,label=$s'$]{sprime}
\end{scope}
\Edge[Direct](s)(u2)
\Edge[Direct](u2)(ui)
\Edge[Direct](ui)(un-1)
\Edge[Direct](un-1)(t)
\Edge[Direct](t)(a1)
\Edge[Direct](a1)(a2)
\Edge[Direct](a2)(ai)
\Edge[Direct](ai)(aK-1)
\Edge[Direct](aK-1)(aK)
\Edge[Direct](aK)(b1)
\Edge[Direct](b1)(b2)
\Edge[Direct](b2)(bi)
\Edge[Direct](bi)(bK-1)
\Edge[Direct](bK-1)(bK)
\Edge[Direct](b2r)(b1r)
\Edge[Direct](bir)(b2r)
\Edge[Direct](bK-1r)(bir)
\Edge[Direct](bK)(bK-1r)
\Edge[Direct](a2r)(a1r)
\Edge[Direct](air)(a2r)
\Edge[Direct](aK-1r)(air)
\Edge[Direct](aKr)(aK-1r)
\Edge[Direct](b1r)(aKr)
\Edge[Direct](uir)(u2r)
\Edge[Direct](un-1r)(uir)
\Edge[Direct](tr)(un-1r)
\Edge[Direct](a1r)(tr)
\Edge[Direct](u2r)(sr)
\Edge[Direct](sr)(sprime)
\Edge[Direct](sprime)(s)
\end{scope}
\end{tikzpicture}

==> img/variablegadget.tex <==
\SetVertexStyle[FillColor=white]
\SetEdgeStyle[Color=black]
\begin{tikzpicture}
  \Vertex[x=0,y=0,label=$v_{i}$,size=0.7]{vi}
  \Vertex[x=1,y=1,label=$t_i^1$,size=0.7]{tif}
  \Vertex[x=2,y=1,label=$\cdots$,style={color=white},size=0.7]{tim}
  \Vertex[x=3,y=1,label=$t_i^{n_i}$,size=0.7]{til}
  \Vertex[x=1,y=-1,label=$f_i^1$,size=0.7]{fif}
  \Vertex[x=2,y=-1,label=$\cdots$,style={color=white},size=0.7]{fim}
  \Vertex[x=3,y=-1,label=$f_i^{p_i}$,size=0.7]{fil}
  \Vertex[x=4,y=0,label=$v_{i+1}$,size=0.7]{vip1}
  \Edge[Direct](vi)(tif)
  \Edge[Direct](tif)(tim)
  \Edge[Direct](tim)(til)
  \Edge[Direct](vi)(fif)
  \Edge[Direct](fif)(fim)
  \Edge[Direct](fim)(fil)
  \Edge[Direct](til)(vip1)
  \Edge[Direct](fil)(vip1)
\end{tikzpicture}


==> tbl/pair_schedule_connectivity.tex <==
\begin{small}
\begin{tabular}{||p{1.3cm}||p{2cm}|p{1.4cm}|p{2cm}|p{3cm}|p{5.4cm}||}
\cline{2-6}
\multicolumn{1}{c||}{} & \multicolumn{5}{c||}{\textbf{Destination}}\\
\hline
\hfil \textbf{Source} & \hfil $c_k\in V^U$ & \hfil $u_k\in V^U$ & \hfil $c_k\in V^L$ & \hfil $l_k\in V^L$  & \hfil $d_k^{l_2}\in V^{\downarrow}_k$\\
\hline\hline
$c_h\in V^U$ & $\begin{array}{ll}S_1^U & \mbox{if $k<h$}\\ T_1^U & \mbox{if $k>h$}\end{array}$  & \centering{$S_k^U$} & \centering{$S_1^U,L_1^{\downarrow},S_1^L$}  & \multicolumn{2}{p{8.4cm}||}{\centering{$S_k^U,T_k^{\downarrow}$}}\\
\hline
$u_h\in V^U$ & \centering{$T_h^U$} & \centering{$T_h^U,T_k^U$} &  \centering{$T_h^{\downarrow},S_h^L$}  & \multicolumn{2}{p{8.4cm}||}{\centering{$\begin{array}{ll}T_k^{\downarrow} & \mbox{if $k=h$}\\ T_h^U,T_k^U,T_k^{\downarrow} & \mbox{if $k\neq h$}\end{array}$}}\\
\hline
$c_h\in V^L$ & \centering{$S_1^L,T^{\uparrow},S_1^U$} & \centering{$S_1^L,T^{\uparrow},S_k^U$} & $\begin{array}{ll}S_1^U & \mbox{if $k<h$}\\ T_1^L & \mbox{if $k>h$}\end{array}$ & \centering{$L_k^B$}  & \multirow{2}{3cm}{\centering{$S_h^L,T^{\uparrow},S_k^U,T_k^{\downarrow}$}}\\
\cline{1-5}
$l_h\in V^L$ & \multicolumn{2}{p{3.4cm}|}{\centering{$S_h^U,L^{\uparrow},S_k^U$}} & \centering{$S_h^L$} & \centering{$T_h^L,T_k^L$} &\\
\hline
$d_h^{l_1}\in V^{\downarrow}_h$ & \multicolumn{2}{p{3.4cm}|}{\centering{$T_h^{\downarrow},S_h^L,T^{\uparrow},S_k^U$}} &  \centering{$T_h^{\downarrow},S_h^L$}  &  $\begin{array}{ll}L_h^{\downarrow} & \mbox{if $k=h$}\\ L_h^{\downarrow},T_h^L,T_k^L & \mbox{if $k\neq h$}\end{array}$ & $\begin{array}{ll}T_h^{\downarrow} & \mbox{if $h=k\wedge l_1<l_2$}\\ T_h^{\uparrow} & \mbox{if $h=k\wedge l_1>l_2$}\\ T_h^{\downarrow},S_h^L,T^{\uparrow},S_k^U,T_k^{\downarrow} & \mbox{if $h\neq k$}\end{array}$\\
\hline\hline
\end{tabular}
\end{small}
